Tensor network square root Kalman filter for online Gaussian process regression

The state-of-the-art tensor network Kalman filter lifts the curse of dimensionality for high-dimensional recursive estimation problems. However, the required rounding operation can cause filter divergence due to the loss of positive definiteness of covariance matrices. We solve this issue by developing, for the first time, a tensor network square root Kalman filter, and apply it to high-dimensional online Gaussian process regression. In our experiments, we demonstrate that our method is equivalent to the conventional Kalman filter when choosing a full-rank tensor network. Furthermore, we apply our method to a real-life system identification problem where we estimate $4^{14}$ parameters on a standard laptop. The estimated model outperforms the state-of-the-art tensor network Kalman filter in terms of prediction accuracy and uncertainty quantification.

==> 0_Parking.tex <==
\subsection{Notes}
\begin{itemize}
    \item synthetic example showing how it works
    \item comparison to existing methods: other automatica paper with Airline data set e.g., WISKI, SVI GP with mini batches (GPflow)
    \item large-scale and high-dimensional data set
\end{itemize}



\subsection{Regression}
Compare to \cite{stanton2021kernel} for Protein, Skillcraft, Elevators, 3DRoad, Powerplant

\subsection{Airline data set}
To compare to existing methods for online GP regression, we perform regression on the airline data set. 
\citet{schurch2020recursive} compares their results to \cite{hensman2013gaussian} by considering mini-batches of $10\thinspace000$ data points over which their iterate multiple times.
Since we consider every sample only once, we can only compare to their RMSE and LML after convergence.

\subsection{Classification}
for classification make banana data set time ordered getting in new values from left to right

check with GPy, GPflow

\subsection{Root covariance approximation}
One data set: show how low-rank approximations impact covariance matrix 
airfoil: compute rmse and final covariance matrix for 10 different splits of data set with Hilbert-GP, with approximations

\subsection{GP basics}
Given a data set of $N_t$ observations, $\x_1,\x_2,\dots,\x_{N_t}$ and $\y=y_1,y_2,\dots,y_{N_t}$, the GP model is given by
\begin{equation}
\begin{aligned}
    y_t &= f(\x_t) + \epsilon_t,\quad\epsilon_t\sim\mathcal{N}(0,\sigma_y^2)\\
    f(\x) &\sim \mathcal{GP}(m(\x),\kappa(\x,\x')),
\end{aligned}
    \label{eq:model}
\end{equation}
where a mean function $m(\cdot)$ and covariance function also called kernel function $\kappa(\cdot,\cdot)$ define the GP, $\sigma_y^2$ denotes the variance of the measurement noise $\boldsymbol\epsilon=\epsilon_1,\epsilon_2,...,\epsilon_{N_t}$, that is assumed to be zero-mean Gaussian and i.i.d., and $\x,\x^\prime\in\mathbb{R}^D$ are $D$-dimensional inputs. 

In GP regression \cite{Rasmussen2006}, the well-known prediction equations for an unseen input $\x_*\in\mathbb{R}^D$ are given by
\begin{equation}\begin{aligned}
f_* \mid \y  &\sim \mathcal{N}\left(\mathbb{E}\left(f_*\right), \mathbb{V}\left(f_*\right)\right), \text { with } \\
\mathbb{E}\left(f_*\right) & =\kk_*^\top\left[\K+\sigma_y^2 \id_{N_t} \right]^{-1} \y\;\; \text{and} \\
\mathbb{V}\left(f_*\right) &=k_{**}-\kk_*^\top\left[\K+\sigma_y^2 \id_{N_t}\right]^{-1} \kk_*, \label{eq:posterior_mP}
\end{aligned}\end{equation}
where the entries of the kernel matrices are computed with $
    [\K]_{tt^\prime} = \kappa(\x_t,\x_{t^\prime})$, $[\kk_*]_t = \kappa(\x_t,\x_*)$ and \mbox{$k_{**} = \kappa(\x_*,\x_*)$}.

The required matrix inversion in \eqref{eq:posterior_mP} is a GP's computational bottleneck of $\mathcal{O}(N_t^3)$ when $N_t$ is large.

Online GP regression with the full GP model \eqref{eq:model} is computationally feasible for a small number of measurements. 
Given the cubic complexity, however, it can quickly become infeasible. 
In addition, for every new measurement, the model needs to be retrained from scratch without being able to take the previous model into account.


%To illustrate our online algorithm, Fig. \ref{fig:watertanks} shows predictions with 95 percent confidence interval for the cascaded water tanks benchmark experiment.
%The validation time-series is predicted after 100, 200 and 992 time steps.
%The figure shows that after seeing 100 measurements, the predictions are not useful, after 200 measurements the predictions are already more accurate, but the confidence interval is quiet large and after 992 measurements, the predictions are quiet good and more certain. \textcolor{orange}{write this a bit nicer. Mention that experiments were done following B-Spline paper.}
%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{Figures/watertanks.png}
%    \caption{Predictions on benchmark data set cascaded water tanks with (a) 100, (b) 200 and (3) 992 measurements as training data.}
%    \label{fig:watertanks}
%\end{figure}


It would be tempting to compute the covariance update given by \eqref{eq:covaupdate} similarly to the mean update by finding a low-rank TT matrix representation for $\Pp_{t-1} - \K_t\Ss_t\K_t^\top$ with the ALS.
This is problematic, however, because the low-rank constraint may cause $\Pp_t$ to lose symmetric positive definiteness.


\subsection{Low matrix rank approximation of covariance matrix}


The resulting thin TTm, which is the new Cholesky factor, $\Ll_t$, has one TT-core with a column index of size $2R$. 
Furthermore, the ranks of the TTm have increased, caused by the summation of two TT matrices.
Since the next time step requires another concatenation between two TT matrices, the algorithm needs some additional steps to stay efficient. \textcolor{orange}{not clear}

The first step is to counteract the increased TT-ranks by applying an algorithm called TT-rounding \cite{Oseledets2011}. 
This algorithm truncates the TT-ranks back to the smaller values and outputs a TTm in site-$d$-mixed canonical form.
The second step is to truncate the TT-core with the column index of size $2R$ back to $R$ \textcolor{orange}{write more intuitively}.
For this, an SVD of the thin TTm, as illustrated in Fig. \ref{fig:thinTT}, needs to be computed.
Since after rounding, the TT matrix is already in site-$d$-mixed canonical form, this can be achieved by computing a singular value decomposition of the $d$th TT-core transformed into a $R_dM_dR_{d+1} \times 2R$ matrix.
Finally, the TT-core is replaced by the truncated $\Ss$-factor computed from the SVD.
The $\V^\top$-factor can be omitted because it cancels out when computing the covariance matrix as shown in \eqref{eq:covfromQR}.





Note that the original ALS algorithm is defined for TTs, so we need to adapt it for TT matrices by transforming them into TTs.
This is possible by combining the row and column index of each TT-core $ \mathbfcal{L}^{(d)}$, transforming the 4-way TTm-cores into 3-way TT-cores, such that it is
\begin{equation}
   \underbrace{R_d\times M_d^\mathrm{row}\times M_d^\mathrm{col} \times R_{d+1}}_{\text{size TTm-core}} \rightarrow \underbrace{R_d\times M_d^\mathrm{row}M_d^\mathrm{col} \times R_{d+1}}_{\text{size TT-core}}.
\end{equation}


\begin{example}[From $\Ll_t\in\mathbb{R}^{M\times 2R}$ to $\Ll_t\in\mathbb{R}^{M\times R}$]
    Assume we have a thin TTm with $D=5$, $M_1=M_2=M_3=M_4=M_5=10$ and $R_2=R_3=R_4=4$ representing $\Ll_t$, where the third core has the column dimension $R=40$. 
    After the update with \eqref{eq:ALScov}, $\mathbfcal{L}^{(3)}\in\mathbb{R}^{4\times10\times 80 \times 4}$ has a doubled column index to the size of $2R$.
    Assuming that the TTm is in site-3-mixed canonical format, an SVD of $\Ll_t$ given by $\mathbf{U}\mathbf{S}\mathbf{V}^\top$, can be computed as follows. 
    First, $\mathbfcal{L}^{(3)}$ is transformed into a matrix of size $R_3M_3R_4\times 2R$.
    Second, an SVD of this matrix is computed given by $\mathbf{U}^{(3)}\mathbf{S}^{(3)}(\mathbf{V}^{(3)})^\top$.
    Third, the third TTm-core is replaced by $\mathbf{U}^{(3)}$ transformed back into a 4-way tensor.
    Now, the thin TTm corresponds to $\mathbf{U}$ and 
    \begin{equation}
        \mathbf{S}=\mathbf{S}^{(3)}\in\mathbb{R}^{R\times R}, \;\;\;\mathbf{V}=(\mathbf{V}^{(3)})^\top\in\mathbb{R}^{R\times 2R}.
    \end{equation}
    Because of \eqref{eq:covfromQR}, the truncated square root factor of size $M\times R$ is simply the thin TTm corresponding to the $\mathbf{U}$ factor with the $S^{(3)}$ factor absorbed into it.
\end{example}


\subsection{Complexity and accuracy}
The computational complexity of the mean update is $\mathcal{O}()$ resulting from the multiplication in TT format between $\Q_{\setminus d, \m_t}^\top$ and the other terms.
Equation \eqref{eq:ALS} can be interpreted as a recursive projection of the least square problem onto a smaller subspace. 
The matrix $\Q_{\setminus d, \m_t}$ acts like a projection matrix, which size determines the subspace onto which the problem is projected.
The accuracy depends on the TT-ranks that are chosen for the initial TT, as well as the approximation of the covariance matrix which is discussed in the next section.

The bottleneck of \eqref{eq:ALScov} is the computation of the term $\Q_{\setminus d,\Ll_t}^\top\K_t\boldsymbol\phi_t\Ll_{t-1}$ as it costs $\mathcal{O}(R_d^4M_d^2)$.
Thus, the computational load will heavily depend on the ranks chosen for the approximation

\subsection{Inverse dynamics of a robotic arm}
In this experiment, we show that the proposed method works for a real-life data set with a large number of input dimensions, as well as a large number of data points.
We use the benchmark industrial robot data set \citep{weigand2022dataset}, which consists of $N=39\thinspace988$ training points and 3636 test points.
To compute the inverse dynamics of the robotic arm, an 18-dimensional input space (position, velocity, and acceleration for 6 joints) is given together with a 6-dimensional output, which are the motor torques for 6 joints.
With $M=4$ basis functions per dimension, the number of parameters are $4^{18}=6.8719\times 10^{10}$.
We consider just one output in our experiment.

%We compare our method to the TNKF which only allows TTm-ranks equal to 1 to guarantee positive (semi-) definiteness.
%We use $R=2$ for our method in the update of $\Ll_t$.
%For the mean update, we use uniform TT-ranks of $R=4$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/kuka.PNG}
    \caption{RMSE and NLL during training. $x$-axis times 400}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
   \includegraphics[width=\columnwidth]{Figures/pred.PNG}
    \caption{Predictions on test data after having trained on $t_1$,$t_2$,$t_3$ data points.}
    \label{fig:enter-label}
\end{figure}

\begin{exmp}[TT-rank increase in covariance update]
The covariance update of the TNKF for a scalar measurement is given by
\begin{equation}
    \Pp_t = \Pp_{t-1} - \mathbf{K}_t\Ss_t\mathbf{K}_t^\top,
\end{equation}
where $\mathbf{P}_{t-1}$ and $\mathbf{P}_t$ are TT matrices, $\mathbf{K}_t$ is a TT, and $\Ss_t$ is a scalar \cite{batselier2017TNKF}.
Say that the TTm-ranks of $\mathbf{P}_{t-1}$ and $\mathbf{K}_t$ are equal to 2, such that the TTm-ranks of $\mathbf{P}_t$ result as follows.
The multiplication in the second term ($\Ss_t$ can be ignored because it is a scalar) causes the TT-ranks to multiply with each other and the addition between the two terms causes the TT-ranks to add onto each other.
Thus, $\mathbf{P}_t$ has TTm-ranks of $2+2\cdot2=6$.
\end{exmp}

\begin{algorithm}
\caption{Transformation of prior on square root covariance factor with Kronecker structure into tall TTm.} \label{alg:kron2thinttm}
    \begin{algorithmic}[1]\onehalfspacing
        \REQUIRE $\Ll_0^{(1)},\Ll_0^{(2)},\cdots, \Ll_0^{(D)}$, maximum TTm-rank $R_\Ll$, column size of tall TTm $R_\mathrm{col}$.
        \ENSURE $\Ll_0$ as thin TTm of size $M\times R_\mathrm{col}$ with TTm-cores $\mathbfcal{L}^{(d)}\in\mathbb{R}^{R_d\times I\times 1 \times R_{d+1}}$ for $d=1,\cdots,d_\mathrm{col}-1,d_\mathrm{col}+1,\cdots D$ and $\mathbfcal{L}^{(d_\mathrm{col})}\in\mathbb{R}^{R_{d_\mathrm{col}}\times I\times R_\mathrm{col} \times R_{d_\mathrm{col}+1}}$.
        \STATE Initialize left-to-right $\mathbf{SV}=1$
        \FOR{$d=1,\dots,d_\mathrm{col}-1$} 
        \STATE Compute $\Ll_\mathrm{tmp}$ as the first $R_\mathrm{col}$ columns with the highest norm of $\Ll_0^{(d)}\otimes\mathbf{SV}$. \label{line:highestnorm}
        \STATE Compute ${R_\Ll}$-truncated SVD \\  $\Ll_\mathrm{tmp}\approx\mathbf{U}^{(d)}\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$.
        \STATE Reshape / permute $\mathbf{U}^{(d)}$ into $\mathbfcal{L}^{(d)}$.
        \STATE Update $\mathbf{SV}=\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$.
        \ENDFOR 
        \STATE Initialize right-to-left $\mathbf{VS}=1$ \\
        \FOR{$d=D,\dots,d_\mathrm{col}+1$}
        \STATE Compute $\Ll_\mathrm{tmp}$ as the first $R_\mathrm{col}$ columns with the highest norm of $\mathbf{SV}\otimes\Ll_0^{(d)}$.
        \STATE Compute ${R_\Ll}$-truncated SVD\\  $\Ll_\mathrm{tmp}^\top\approx\mathbf{U}^{(d)}\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$.
        \STATE Reshape / permute $(\mathbf{U}^{(d)})^\top$ into $\mathbfcal{L}^{(d)}$.
        \STATE Update $\mathbf{VS}=\mathbf{V}^{(d)}\mathbf{S}^{(d)}$.
        \ENDFOR 
        \STATE Compute $\mathbfcal{L}^{(d_\mathrm{col})}$ by reshaping / permuting first $R_\mathrm{col}$ columns with highest norm of\\ $\mathbf{VS}^\top\otimes \Ll_0^{(d_\mathrm{col})}\otimes \mathbf{SV}$.
    \end{algorithmic}
\end{algorithm}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/watertanks_predictions.png}
    \caption{Predictions at three different time instances}
    \label{fig:predtanks}
\end{figure}

In addition, in Fig.\ \ref{fig:predtanks} we visualize the predictive mean with uncertainty bound for our method with $R_\Ll=4$ after having seen 100, 200 and 922 data points.
The figure shows that with more observed data points the mean prediction becomes better and the certainty becomes higher. 

\begin{figure}
    \centering
    \input{Figures/term2_lowrank_notdcol}
    \caption{Visual depiction for computing \eqref{eq:term2_eq2} for $d\neq d_\mathrm{col}$ resulting in a 4-way tensor of size $R_\Ll\times I\times 1\times R_\Ll$.}
    \label{fig:term2_lowrank}
\end{figure}

To compute \eqref{eq:sqrt} in TN format, we need to to concatenate matrices in TN format.
To illustrate how this works, take the following definition.
\begin{defn}\textbf{(Horizontal Concatenation of two TT matrices)}
Take $\mathbf{A}\in\mathbb{R}^{M\times M}$ and $\mathbf{B}\in\mathbb{R}^{M\times 1}$ as two TT matrices.
Then, the concatenation of $\mathbf{A}$ and $\mathbf{B}$ is given by
\begin{equation}
    \begin{aligned}
        \begin{bmatrix}\mathbf{A}&\mathbf{B} \end{bmatrix}=&\begin{bmatrix} 1&0 \end{bmatrix} \otimes \mathbf{A} + \begin{bmatrix} 0&1 \end{bmatrix}\otimes \begin{bmatrix}
            1&\boldsymbol{0}_{M-1}
        \end{bmatrix} \otimes \mathbf{B},
    \end{aligned} \label{eq:eg_summation}
\end{equation}
where both summands are of size $M\times 2M$.
\label{def:concat}
\end{defn}


\section{Related work}
Our work relates to literature about scalable GP approximations, recursive estimation with low-rank covariance matrices, and scalable low-rank TN GP regression models.

\textcolor{orange}{Scalable GP approximations:}
While numerous approximations exist to address scalability in batch settings e.g.\ \cite{wilson2015kernel,quinonero2005unifying,HilbertGP}, there is a notable scarcity of research focusing on scalable online inference methods for GPs, despite growing demand in this area.
Especially for large-scale and high-dimensional data there are not a lot of methods and the existing ones require dimensionality reduction to deal with a high number of input features \cite{stanton2021kernel}.

Among the most known GP approximations are sparse GPs \cite{quinonero2005unifying} with their extension for inducing inputs on a grid \cite{wilson2015kernel}, and Hilbert-space methods for reduced-rank GPs \cite{HilbertGP}.
Both approximations have an online version, where the parametric GP model is updated recursively with new incoming measurements.

\begin{itemize}
    \item online Hilbert-space method for reduced-rank GP: \cite{sarkka2013spatiotemporal} \textcolor{orange}{what to cite? sensor fusion papers} [...] formulate the reduced-rank model as a Kalman filter measurement update which costs $\mathcal{O}(M^2)$
    \item \cite{bui2017streaming} are the first to introduce sparse GP approximations for streaming data.
    \item Online GP with inducing inputs on a grid \cite{stanton2021kernel} use a combination of structured kernel interpolation and Woodbury identity to achieve constant-time updates $\mathcal{O}(1)$ for $N$ data points and $\mathcal{O}(M^2)$ for $M$ inducing inputs.
    However, they need to perform dimensionality reduction on high-dimensional data sets. 
    \item Recursive GP algorithm \cite{schurch2020recursive}: Similar to Hensman they compute the posterior using mini-batches (around 10'000 samples) and iterate over them multiple times. They also do hyperparameter optimization in this way
\end{itemize}

\textcolor{orange}{Recursive estimation with low-rank covariance matrices:} Regarding recursive estimation with low-rank covariance matrices, this work relates to \cite{bonnabel2012geometry,schmidt2023rank} which update their covariance matrices on a low-rank manifold.
\textcolor{orange}{find more and relate to this work}


\textcolor{orange}{Scalable low-rank TN models for GP approximation:} \cite{izmailov2018scalable,nickson2015blitzkriging,hensman2017variational}, where the covariance matrices of the inducing inputs posterior distribution are represented with Kronecker products that can be related to TNs.

In e.g.\ \cite{dolgov2014alternating}, the ALS is used to invert a matrix in TTm format.


\subsubsection{Moving of index to change augmented TTm-core}
During the ALS, $\Ll_t$ is computed in terms of a TTm of size $M\times 2M$ with row indices of size $I$ and column index of size $J$ and one of size $2J$.
The augmented TTm-core with the column index of size $2J$ is updated, and after each update, the index of size two is moved to the next TTm-core to be updated.
This is because, in some cases, higher accuracy can be achieved compared to not always updating the augmented TTm-core. 
However, for general recommendations on whether to move the index or not, more analysis is necessary.
The implementation of moving the index from the $d$th to the $(d+1)$th TTm-core is given in Algorithm \ref{alg:prop} with illustrations in Fig.\ \ref{fig:indexprop}.
The computations are analog for moving the index from the $d$th to $(d-1)$th TTm-core.
The algorithm's inputs are the currently augmented TTm-core and the TTm-core, where the index of size two is moved. 
The essence of the algorithm is to divide the currently augmented TTm-core from the index of size two by using the SVD and then moving the index to the next TTm-core.

\begin{figure}
    \centering
    \input{Figures/indexprop}
    \caption{Moving of column index from augmented TTm-core to the next. (a) TTm where $d$th TTm-core (highlighted with light green box) is augmented and $(d+1)$th TTm-core (blue node) is to-be-augmented TTm-core. (b) $d$th TTm-core transformed into a matrix (highlighted in light green). (c) SVD of the matrix from (b) ($\textbf{U}^{(d)}$-factor is the green node and $\textbf{S}^{(d)}$- and $\textbf{V}^{(d)}$-factor are yellow nodes). (d) Replacing $d$th TTm-core with $\mathbf{U}^{(d)}$ (green node) and combining $\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$ (yellow node). (e) Absorbing $\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$ into $(d+1)$th TTm-core resulting in new augmented TTm-core (highlighted in the light blue box).}
    \label{fig:indexprop}
\end{figure}

\begin{algorithm}
\caption{Moving of index from $d$th TTm-core to $(d+1)$th}\label{alg:prop}
    \begin{algorithmic}[1]\onehalfspacing
    \REQUIRE $\mathbfcal{L}_t^{(d)} \in \mathbb{R}^{R_{d}\times I\times 2J \times R_{d+1}}$ (current augmented TTm-core),
    $\mathbfcal{L}_t^{(d+1)}\in \mathbb{R}^{R_{d+1}\times I\times J \times R_{d+2}}$.
    \ENSURE $\mathbfcal{L}_t^{(d)} \in \mathbb{R}^{R_{d}\times I\times J \times R_{d+1}}$,\\ \mbox{$\mathbfcal{L}_t^{(d+1)}\in \mathbb{R}^{R_{d+1}\times I\times 2J \times R_{d+2}}$} (newly augmented TTm-core).
        \STATE Reshape / permute $\mathbfcal{L}_t^{(d)}$ into matrix of size $R_{d}IJ \times 2R_{d+1}$ \mbox{(Fig.\ \ref{fig:indexprop}(b))}.
        \STATE Compute SVD of matrix from line 1 given by $\mathbf{U}^{(d)}\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$ \mbox{(Fig.\ \ref{fig:indexprop}(c))}.
        \STATE Reshape $\mathbf{U}^{(d)}\in\mathbb{R}^{R_{d}IJ\times R_{d+1}}$ into TTm-core $\mathbfcal{L}_t^{(d)} \in \mathbb{R}^{R_{d}\times I\times J \times R_{d+1}}$ \mbox{(Fig.\ \ref{fig:indexprop}(d))}.
        \STATE Absorb $\mathbf{S}^{(d)}(\mathbf{V}^{(d)})^\top$ into $(d+1)$th TTm-core such that $\mathbfcal{L}_t^{(d+1)}\in \mathbb{R}^{R_{d+1}\times I\times 2J \times R_{d+2}}$ \mbox{(Fig.\ \ref{fig:indexprop}(e))}.
    \end{algorithmic}
\end{algorithm} 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/KFcomparison.png}
    \caption{Comparison between Kalman filter and square/tall $\Ll_t$ for full rank and with low-rank approximation for $D=3$. The curves for the Kalman filter lie on top of the curves for $R_\mathrm{col}=64$.}
    \label{fig:KFcomparison}
\end{figure}

For $R_\mathrm{col}=64$ and all TTm-ranks of the tall $\Ll_t$ maximum equal to 16, there is no difference to the Kalman filter. 
This is because, firstly, the TT and TTm are full-rank. 
Secondly, the number of columns $R_\mathrm{col}$ are equal to the number of columns; and thirdly, the QR-step, as described in section \ref{sec:QRstep_tall} is exact. 
Thus, there is no approximation made.

For the dark orange and green curve, $R_\mathrm{col}$ is a smaller value than the full matrix rank, but all $R_\w$ and $R_\Ll$ are kept the same.
The performance is lower because the $\Pp_t$ is assumed to have a low matrix rank, which is not necessarily true.
Thus, it will heavily depend on the data if the tall $\Ll_t$ approximation is suitable.
Also note that the TNSRKF with a tall $\Ll_t$ requires the choice of $R_\w$ and a maximum value for $R_\Ll$, which results in further approximations.

The violet curve is the predictions computed with the TNSRKF with a square $\Ll_t$. 
Although $\w_t$ and $\Ll_t$ are both full rank, the performance is lower than the Kalman filter.
This is because the QR-step described in section  \ref{sec: QRstep_square} is not exact.
The performance is worse for lower ranks, but again, the data will determine if low-rank approximations are suitable.

==> 3_Methods_new.tex <==
\clearpage
\section{Method}
We now propose our method that combines efficient TN-based tools with the SRKF formulation for online GPs.
All computations are summarized in Algorithm \ref{alg:onlineregression}.

\subsection{Update of weight mean}
For updating the mean with a new minibatch of $B$ samples $\y_t\in\mathbb{R}^B$, we compute \eqref{eq:meanupdate} in TN format.
In the original tensor-based KF \cite{batselier2017TNKF}, the summands of equation \eqref{eq:meanupdate} are summed together in TT format.
Summation increases the TT-ranks which can be counteracted by an additional step called TT-rounding \cite{Oseledets2011}, an operation that can become costly. 

In contrast, we apply a commonly-used optimization algorithm from the tensor community, called the alternating linear scheme (ALS) \cite{Rohwedder2012,Rohwedder2013}.
The optimization problem to be solved is given by
\begin{equation}
\begin{aligned}
    \min_{\m_t} &\| \left[\m_{t-1} + \K_t(\y_t-\boldsymbol\Phi_t \m_{t-1})\right] - \m_t \|_\mathrm{F}^2\\
    & \text{s.t.}\;\; \m_t\;\;\text{being a low-rank TT}, \label{eq:optproblem}
\end{aligned}
\end{equation}
where the subscript F stands for the Frobenius norm.
The ALS solves \eqref{eq:optproblem} in the style of a block-coordinate descent by computing smaller optimization problems sequentially.
In this way, multiple smaller and less computationally heavy optimization problems are solved.
This is achieved by updating the TT core by core while keeping all cores fixed that are not currently updated.
Updating each TT-core once is called a sweep and for the online scenario, one sweep is usually sufficient for the residual of \eqref{eq:optproblem} to converge.

Making use of the site-$d$-mixed canonical format from definition \ref{def:sitek}, the TT representing the mean can be written $\m_t=\Q_{\setminus d,\m_t}\m_t^{(d)}$, where \mbox{$\Q_{\setminus d,\m_t}\in\mathbb{R}^{M\times R_dM_dR_{d+1}}$} is an orthogonal matrix computed from all TT-cores except the $d$th, indicated by the setminus $d$ in the subscript, and $\m_t^{(d)}\in\mathbb{R}^{R_dM_dR_{d+1}}$ is the vectorization of the $d$th TT-core.

In this way, \eqref{eq:optproblem} can be rewritten as $D$ different optimization problems, each of which is given by 
\begin{equation}
    \min_{\m_t^{(d)}} \| \Q_{\setminus d, \m_t}^\top[\m_{t-1} + \mathbf{K}_t(\y_t-\boldsymbol\Phi_t \m_{t-1})] - \m_t^{(d)} \|_\mathrm{F}^2. \label{eq:ALS}
\end{equation}
Here, $\m_{t-1}$ is the mean in TT-format computed in the last time step that serves as prior for the current time step.
Note that now it is optimized over one TT-core and not the entire tensor train.

\subsubsection*{Implementation}
At $t=0$, Algorithm \ref{alg:onlineregression} requires initializations.
The initial guess for the TT representing $\m_t$ is randomly sampled from a zero-mean Gaussian and transformed into a site-$d$-mixed canonical format. 
Since $\m_t^{(d)}$ is the first core to-be-updated, the algorithm just needs $\Q_{\setminus d, \m_0}$ as an input.
Note that this initialization is for $\m_{t=1}$, which is different from the prior for the mean $\m_{t=0}$.
The following Lemma explains how the prior mean $\m_0$ with the assumption to be zero mean is initialized in TT format.

\begin{lemma}[Zero-mean prior in TT format \cite{Batselier2019extended}]
    Given the zero-mean prior assumption $\m_0=\boldsymbol{0}_M$, an initial TT for the ALS that fulfils that assumption is given by a TT in site-$d$-mixed canonical format where $\Q_{\setminus d,\m_0}$ is a random orthogonal matrix, meaning that all cores except the $d$th are randomly initialized and the orthogonalized and the $d$th core contains only zeros such that $\m_0^{(d)}=\boldsymbol{0}_{M_d}$. \label{lem:zmprior}
\end{lemma}

Regarding the efficient implementation of \eqref{eq:ALS}, both $\K_t$ and $\boldsymbol{\Phi_t}$ are thin TT matrices as illustrated in Fig. \ref{fig:thinTT}. 
To efficiently compute this expression, take the following example.

\begin{example}
    Take $\Q_{\setminus d, \m_t}^\top\in\mathbb{R}^{50\times 10^8}$ and $\m_t,\K_t\in\mathbb{R}^{10^8\times 1}$. In addition, take  $y_t-\boldsymbol\phi_t \m_{t-1}=v_t\in\mathbb{R}$ as a scalar.
    By first multiplying over the large dimension of $10^8$ in TN format in $\Q_{\setminus d, \m_t}^\top \m_t$ and $\Q_{\setminus d, \m_t}^\top \K_t v_t$, and then summing two vectors of size $50$, the expression in \eqref{eq:ALS} can be efficiently computed.
\end{example}

\subsubsection*{Complexity and accuracy}
The computational complexity of the mean update is $\mathcal{O}()$ resulting from the multiplication in TT format between $\Q_{\setminus d, \m_t}^\top$ and the other terms.
Equation \eqref{eq:ALS} can be interpreted as a recursive projection of the least square problem onto a smaller subspace. 
The matrix $\Q_{\setminus d, \m_t}$ acts like a projection matrix, which size determines the subspace onto which the problem is projected.
The accuracy depends on the TT-ranks that are chosen for the initial TT, as well as the approximation of the covariance matrix which is discussed in the next section.


\section{These paragraphs need to go somewhere}
Regarding computational complexity, the KF update for the mean \eqref{eq:meanupdate} and covariance \eqref{eq:covaupdate} require $\mathcal{O}(M)$ and $\mathcal{O}(M^2)$, respectively.
The square-root update requires a QR-decomposition of a tall matrix, which costs $\mathcal{O}(MR^2)$.
For a regression problem with high-dimensional input features, $M$ can grow exponentially with the dimensionality and can thus cause a prohibitive computational cost.

To initialize the SRKF, the prior on the weights \mbox{$\w_0=\mathcal{N}(\m_0,\Pp_0)$} depends on the choice of problem that we would like to solve.
For Gaussian process regression with the squared exponential kernel, it is $\m_0=\boldsymbol{0}$ and $\Pp_0=\boldsymbol{\Lambda}$, where $\boldsymbol{\Lambda}$ is a diagonal matrix with exponentially decaying values on the diagonal \cite{HilbertGP}.
For Volterra system identification, we also set $\m_0=\boldsymbol{0}_M$ and $\Pp_0=\lambda\id_M$, with $\lambda$ denoting the Tykonov regularization parameter.

==> old_1_1_Introduction_commented.tex <==
\section{Introduction}
In a time where data-driven AI models are trained on an exponentially growing amount of data, it is crucial the models can be adapted to newly observed data without the need for retraining from scratch.
These online or recursive settings can be found in many fields including system identification \textcolor{orange}{[ ]}, sensor fusion \cite{viset2022extended,solin2018modeling}, robotics \cite{nguyen2008local}, and machine learning \textcolor{orange}{[ ]}.

Bayesian recursive algorithms are well-suited for these applications, allowing for model updates based on priors computed from previously seen data. 
However, widely-used Gaussian processes \cite{Rasmussen2006} (GPs) encounter difficulties in online settings due to the cubic cost of inference with the number of all observed points each time there is new data.


In the weight-space view of GPs \citep[Chapter 2]{Rasmussen2006}, the GP model is written in terms of a parametric Bayesian linear regression model, where the cost is $\mathcal{O}(NM^2)$, with $M$ being the number of parameters.
The advantage of this setting is that it is possible by sequentially updating the posterior distribution \mbox{$p(\w_t\mid\y_{1:t})$} and using it as the prior for the next update \cite{sarkka2023bayesian}, like in the measurement update of a Kalman filter.
In this case, the cost becomes $\mathcal{O}(M^2)$ for every time step, independent of how many data points have been already observed.






Given a data set of $N$ scalar observations, $\y=y_1,...,y_t,...,y_{N}$, a GP model is given by
\begin{equation}
\begin{aligned}
    y_t &= f(\x_t) + \epsilon_t,\quad\epsilon_t\sim\mathcal{N}(0,\sigma_y^2)\\
    f(\x_t) &= \mathcal{GP}(m(\x_t),\kappa(\x_t,\x_t'))
\end{aligned}
    \label{eq:model}
\end{equation}
where $m(\cdot)$ and $\kappa(\cdot,\cdot)$ are the mean and kernel function, respectively, $\x_t,\x_t^\prime\in\mathbb{R}^D$ are $D$-dimensional inputs, $\sigma_y^2$ denotes the variance of the measurement noise and $\boldsymbol\epsilon=\epsilon_1,...,\epsilon_t,...,\epsilon_{N}$, assumed to be i.d.d. and zero-mean Gaussian.
Performing inference with \eqref{eq:model} involves an inversion of a matrix of size of the observations, thus a complexity of $\mathcal{O}(N^3)$.
In an online setting, the number of observations grow and each time step $t$ requires a cubic cost in $N$, which can cause a computational bottleneck.

A more computationally efficient approach to online GPs is trough the weight-space view, where the GP model is written in terms of a parametric Bayesian linear regression model \citep[Chapter 2]{Rasmussen2006} given by
\begin{equation}
    y_t = \boldsymbol{\phi}_t^\top \w_t + \epsilon_t,\quad\epsilon_t\sim\mathcal{N}(0,\sigma_y^2),
    \label{eq:parammodel}
\end{equation}
where $\boldsymbol{\phi}_t=\boldsymbol{\phi}(\x_t)$ is a function that maps the input vector to a feature space evaluated at input $\x_t$, and $\w_t\in\mathbb{R}^M$ is a weight vector with prior $\w_0\sim\mathcal{N}(\hat\w_0,\mathbf{P}_0)$.
The parametric model \eqref{eq:parammodel} allows for an online algorithm which updates the weights $\w$ sample by sample at a cost of $\mathcal{O}(M^2)$. 














Being a kernel method, GPs require a kernel function which determines which types of functions can be modeled, e.g. with regard to smoothness.
Commonly-used kernels in GP regression are product kernels, which require the number of basis functions $\boldsymbol{\phi}$ in model \eqref{eq:parammodel} to grow exponentially with the number of input dimensions, giving rise to the curse of dimensionality.






















For both the basis functions of the squared exponential kernel, and the Volterra kernel, the curse of dimensionality has been lifted in tensor network format for the batch setting by \cite{batselier2017VoleterrALS} and \cite{wesel2021large}, respectively.

For the online setting, \cite{batselier2017TNKF,Batselier2019extended} give a solution in terms of the tensor-networked Kalman filter (TNKF).
While the TNKF lifts the curse of dimensionality it has a major drawback: 
Due to a TN specific operation called rounding, which is crucial for the effciency of the algorithm, the covariance update can suffer from the loss of positive definiteness.
We solve this issue by updating the square root of the covariance matrix in tensor network (TN) format.

Our main contribution is a tensor-networked square root Kalman filter (SRKF) for online GPs regression for many data points and high-dimensional input features in a computationally more stable way than previously suggested work. 


TNKF high level what is does and drawbacks: tn specific operations
story line a bit hidden, 
make urgency clear!!
its not a straight forward thing





%Another motivation: online methods because like in stochastic gradient descent not all data can be handled at once.

==> temp.tex <==
\begin{equation}
    \begin{aligned}
        \underbrace{\mathbf{l}_t^{(3)}}_{3200\times1} =  & \begin{bmatrix}1&0\end{bmatrix}^\top\otimes \left(\underbrace{\begin{bmatrix}\id_M&\boldsymbol{0}_M\end{bmatrix}\mathbf{H}_{d,t}^\top}_{1600\times10^{10}} \underbrace{\operatorname{vec}\left(\Ll_{t-1}\right)}_{10^{10}\times 1}\right)\\
        -& \begin{bmatrix}1&0\end{bmatrix}^\top\otimes\left(\underbrace{\begin{bmatrix}\id_M&\boldsymbol{0}_M\end{bmatrix}\mathbf{H}_{d,t}^\top}_{1600\times10^{10}} \underbrace{\operatorname{vec}\left(\K_t\boldsymbol\phi_t^\top\Ll_{t-1}\right)}_{10^{10}\times 1}\right)\\
        + & \begin{bmatrix}0&1\end{bmatrix}^\top\otimes\left(\underbrace{\begin{bmatrix}\boldsymbol{0}_M&\id_M\end{bmatrix}\mathbf{H}_{d,t}^\top }_{1600\times 10^{10}} \underbrace{\operatorname{vec}\left(\begin{bmatrix}1&\boldsymbol0\end{bmatrix}\otimes\sigma_y\K_t\right)}_{10^{10}\times 1}\right).
    \end{aligned}\label{eq:threeterms}
    \end{equation}

==> tmp.tex <==
\begin{algorithm}
\caption{QR-step for thin and square $\Ll_t$}\label{alg:retruncate}
    \begin{algorithmic}[1]\onehalfspacing
    \REQUIRE TTm for $\Ll_t$ in site-$d_\text{col}$-mixed canonical format with $\mathbfcal{L}^{(d_\text{col})}$ of size $R_{d_\text{col}}\times M_{d_\text{col}}\times 2J \times R_{d_\text{col}+1}$ 
    \ENSURE TT for $\Ll_t$ with $\mathbfcal{L}^{(d_\text{col})}$ of size \\ \;\;\;\;\;\;\;$R_{d_\text{col}}\times M_{d_\text{col}}\times J\times R_{d_\text{col}+1}$ 
        \STATE Transform $\mathbfcal{L}^{(d_\text{col})}$ of size $R_{d_\text{col}}\times M_{d_\text{col}}\times 2J \times R_{d_\text{col}+1}$ into matrix of size $JM_{d_\text{col}}R_{d_\text{col}+1}\times 2J$.
        \STATE Compute $J$-truncated SVD of matrix from line 1 given by $\mathbf{U}^{(d_\text{col})}\mathbf{S}^{(d_\text{col})}(\mathbf{V}^{(d_\text{col})})^\top$
        \STATE Transform $\mathbf{U}^{(d_\text{col})}\mathbf{S}^{(d_\text{col})}$ of size $R_{d_\text{col}}M_{d_\text{col}}R_{d_\text{col}+1}\times J$ into tensor of size $J\times M_{d_\text{col}}\times J\times R_{d_\text{col}+1}$.
        \STATE Replace $\mathbfcal{L}^{(d_\text{col})}$ by tensor from line 4.
    \end{algorithmic}
\end{algorithm}
